No-Rainbow Problem and the Surjective Constraint Satisfaction Problem

The Surjective Constraint Satisfaction Problem (SCSP) is the problem of deciding whether there exists a surjective assignment to a set of variables subject to some specified constraints, where a surjective assignment is an assignment containing all elements of the domain. In this paper we show that the most famous SCSP, called No-Rainbow Problem, is NP-Hard. Additionally, we disprove the conjecture saying that the SCSP over a constraint language $\Gamma$ and the CSP over the same language with constants have the same computational complexity up to poly-time reductions. Our counter-example also shows that the complexity of the SCSP cannot be described in terms of polymorphisms of the constraint language.

==> Preamble.tex <==
The \emph{Constraint Satisfaction Problem (CSP)} is the problem of deciding whether there is an assignment to a set of variables
subject to some specified constraints. 
In this paper we consider only CSP over finite domains.
The general CSP is known to be NP-complete \cite{Num26, Num30}; however, certain restrictions
on the allowed form of constraints involved may ensure tractability (solvability in polynomial time)
\cite{Num4,Num20,Num22,Num23,CSPconjecture,BulatovAboutCSP}.
Below we provide a formalization to this idea.

For a set of relations $\Gamma\subseteq R_{A}$ by $\CSP(\Gamma)$
we denote the Constraint Satisfaction Problem where all
the constraint relations are from $\Gamma$.
The set $\Gamma$ is called \emph{a constraint language}.
Another way to formalize the Constraint Satisfaction Problem is
via conjunctive formulas.
Every $h$-ary relation on $A$ can be viewed as
a predicate, that is, a
mapping $A^{h}\rightarrow \{0,1\}$.
Suppose $\Gamma\subseteq R_{A}$, then $\CSP(\Gamma)$ is the following decision problem:
given a formula
$$\rho_{1}(v_{1,1},\ldots,v_{1,n_{1}})
\wedge
\dots
\wedge
\rho_{s}(v_{s,1},\ldots,v_{s,n_{s}}),$$
where $\rho_{1},\dots,\rho_{s}\in \Gamma$, 
and $v_{i,j}\in \{x_{1},\dots,x_{n}\}$ for every $i,j$;
decide whether this formula is satisfiable.


We say that an operation
$f\colon A^{n}\to A$ \emph{preserves} the relation $\rho\in R_{A}$ of arity $m$
if for any tuples $(a_{1,1},\ldots,a_{1,m}),\dots,(a_{n,1},\ldots,a_{n,m})\in \rho$
the tuple
$(f(a_{1,1},\ldots,a_{n,1}),\ldots,f(a_{1,m},\ldots,a_{n,m}))$ is in $\rho$.
We say that an operation \emph{preserves a set of relations $\Gamma$} if it preserves every relation in $\Gamma$.
A mapping $f:A\to A$ is called \emph{an endomorphism} of $\Gamma$ if it preserves $\Gamma$. %every relation $\rho\in \Gamma$.
%It can be shown

\begin{thm}\label{coreHasSameComplexity}\cite{jeavons1998algebraic}
Suppose $\Gamma\subseteq R_{A}$.
If $f$ is an endomorphism of $\Gamma$, %$f:A\to A$ preserves every relation of $\Gamma$,
then $\CSP(\Gamma)$ is polynomially reducible to $\CSP(f(\Gamma))$ and vice versa,
where $f(\Gamma)$ is a constraint language with domain $f(A)$
defined by $f(\Gamma) = \{f(\rho)\colon \rho\in \Gamma\}$.
\end{thm}

A constraint language is \emph{a core} if every endomorphism of $\Gamma$ is a bijection.
It is not hard to show that if $f$ is an endomorphism of $\Gamma$ with minimal range,
then $f(\Gamma)$ is a core. Another important fact is that we can add all
singleton unary relations to a core constraint language
without increasing the complexity of its $\CSP$.
By $\sigma_{=a}$ we denote the unary relation $\{a\}$.

\begin{thm}\label{addingIdempotency}\cite{CSPconjecture}
Let $\Gamma\subseteq R_{A}$ be a core constraint language, and
$\Gamma' = \Gamma\cup \{\sigma_{=a}\mid a\in A\}$.
Then $\CSP(\Gamma')$ is polynomially reducible to $\CSP(\Gamma)$.
\end{thm}
Therefore, to prove Conjecture~\ref{FederVardiConj} it is sufficient to consider only the case when
$\Gamma$ contains all unary singleton relations.
In other words, all the predicates $x = a$, where $a\in A$, are in the constraint language $\Gamma$.

In \cite{Schaefer} Schaefer
classified all tractable constraint languages over two-element
domain. In \cite{BulatovForThree} Bulatov generalized the result for three-element domain.
His dichotomy theorem was formulated in terms of a $G$-set.
Later, the dichotomy conjecture was formulated in several different forms (see \cite{CSPconjecture}).

The result of Mckenzie and Mar{\'o}ti~\cite{miklos} allows us to formulate the dichotomy conjecture in the following nice way.
An operation $f$ on a set $A$ is called \emph{a weak near-unanimity operation (WNU)} if it satisfies 
%$f(x,x,\ldots,x) = x$ and
$f(y,x,\ldots,x) = f(x,y,x,\ldots,x) = \dots = f(x,x,\ldots,x,y)$
for all $x,y\in A$.
An operation $f$ is called \emph{idempotent} if $f(x,x,\ldots,x) = x$ for all $x\in A$.

\begin{conj}\label{mainconj}
Suppose $\Gamma\subseteq R_{A}$ is a finite set of relations.
%$\{\sigma_{=a}\mid a\in A\} \subseteq \Gamma$.
Then $\CSP(\Gamma)$ can be solved in polynomial time if there exists a WNU
preserving $\Gamma$;
$\CSP(\Gamma)$ is NP-complete otherwise.
\end{conj}

It is not hard to see that
the existence of a WNU preserving $\Gamma$ is equivalent to the existence of
a WNU preserving a core of $\Gamma$,
and also equivalent to
the existence of an idempotent WNU preserving the core.
Hence, Theorems~\ref{coreHasSameComplexity} and \ref{addingIdempotency}
imply that it is sufficient to prove Conjecture~\ref{mainconj}
for a core and an idempotent WNU.

One direction of this conjecture follows from \cite{miklos}.
\begin{thm}\label{MiklosMckenzie}\cite{miklos}
Suppose $\Gamma\subseteq R_{A}$ and 
$\{\sigma_{=a}\mid a\in A\} \subseteq \Gamma$.
If there exists no WNU
preserving $\Gamma$, then $\CSP(\Gamma)$ is NP-complete.
\end{thm}

%%As it follows from Theorem~\ref{addingIdempotency} and Theorem~\ref{MiklosMckenzie},
%%to prove Conjecture~\ref{mainconj} it remains to
%%find a polynomial algorithm for constraint languages preserved by an idempotent WNU.

The dichotomy conjecture was proved for many special cases:
for CSPs over undirected graphs \cite{hell1990complexity},
for CSPs over digraphs with no sources or sinks \cite{barto2009csp},
for constraint languages containing all unary relations~\cite{bulatov2003conservative},
and many others.
%Recently, Rafiey, Kinne, and Feder
%announced the proof of the general case~\cite{PossibleProofCSP}.
More information about the algebraic approach to CSP can be found in \cite{bartopolymorphisms}.

In this paper we present an algorithm that
solves $\CSP(\Gamma)$ in polynomial time if $\Gamma$ is preserved by an idempotent WNU,
and therefore prove the dichotomy conjecture.

\begin{thm}
Suppose $\Gamma\subseteq R_{A}$ is a finite set of relations.
%$\{\sigma_{=a}\mid a\in A\} \subseteq \Gamma$.
Then $\CSP(\Gamma)$ can be solved in polynomial time if there exists a WNU
preserving $\Gamma$;
$\CSP(\Gamma)$ is NP-complete otherwise.
\end{thm}

Another proof of the dichotomy conjecture was announced by Andrei Bulatov~\cite{BulatovProofCSP,BulatovProofCSPFOCS}.
Even though both algorithms appeared at the same time, they are significantly different. 
Bulatov's algorithm uses full strength of the few subpowers algorithm \cite{idziak2010tractability}, 
uses Maroti's trick for trees on top of Mal'tsev \cite{maroti2011tree}, 
while this one just checks some local consistency and solves linear equations over prime fields. 
Also Bulatov's algorithm works for infinite constraint languages, which is not the case for the algorithm presented in this paper.
But its slight modification works even for infinite constraint languages \cite{zhuk2018modification}.


The paper is organized as follows.
In Section~\ref{ZFourExample} we explain the algorithm informally and 
give an example showing how the algorithm works
for a system of linear equations in $\mathbb Z_{4}$.
In Section~\ref{Definition} we give main definitions,
in Section~\ref{Algorithm}
we give a formal description of the algorithm
showing a pseudocode for most functions
and explain the meaning of every function.
In Section~\ref{CorretnessSection} we formulate all theorems 
that are necessary to prove the correctness of the algorithm.
Then, we prove that on every algebra (domain) with
a WNU operation 
there exists a subuniverse of one of four types, which is the main ingredient of the algorithm. 
Additionally, in this section we prove that 
some functions of the algorithm work properly 
and the algorithm actually works in polynomial time.

In Section~\ref{DefinitionSection} we give the remaining definitions.
The proof of the main theorems is divided into three sections.
In Section~\ref{AbsCenterPCLinear} we study  properties of
subuniverses of each of four types (absorbing, central, PC, and linear subuniverses).
In Section~\ref{AuxStatements} we prove all the auxiliary statements, and in the last section we prove the main theorems of this paper formulated in Section~\ref{CorretnessSection}.

In Section~\ref{ConclusionsSection}, 
we discuss open questions
and consequences of this result.
In particular, we consider generalizations 
of the CSP such as Valued CSP, Infinite Domain CSP, Quantified CSP, Promise CSP and so on.



%A CSP instance $\Theta$ is called \emph{1-consistent} if
%for any constraint $(t,R)$ the relation $R$ is subdirect.

%%%if the set of all variables that appears in $\Theta$
%%%can be divided into two sets $X_{1}$ and $X_{2}$ such that
%%%any constraint of $\Theta$ either has variables only from $X_{1}$
%%%or only from $X_{2}$.
%%%
%%%A CSP instance is called \emph{linked} if
%%%for any $i$ and $a,b\in A_{i}$ there exists a path $x_{i}-C_{1}-x_{i_1}-\dots-\dots-x_{i_l}-C_{l+1}-x_{i}$
%%%from $a$ to $b$.

%%A CSP instance $\Theta$ is called \emph{irreducible} if for
%%any nonlinked nontrivial subinstance $\Theta'$
%%,any variable $x_{i}$ that appears in $\Theta'$,
%%and any $a\in A_{i}$ we have a solution of $\Theta'$ with $x_{i} = a$.
%
%\section{Algorithm}
%
%Function $\CSP(\Theta)$
%    $PathConsistency(\Theta)$
%    $Irreducible(\Theta)$
%    If exists a proper binary absorbing set on $A_{i}$
%        $\overline D := MinimalAbsorbingSets(\Theta)$;
%        $\Theta' := Reduction (\Theta;\overline D);$
%        return $\CSP(\Theta;\overline D')$
%    end if;
%
%    If exists a proper center on $A_{i}$
%        $\overline D := MinimalCentralSets(\Theta)$;
%        $\Theta' := Reduction (\Theta;\overline D);$
%        return $\CSP(\Theta;\overline D')$;
%    end if;
%
%    If $A_{i}/\sigma$ is polynomially complete for some  $i$  and a congruence $\sigma$ on $A_{i}$
%        $\overline D := MinimalPCClasses(\Theta)$;
%        $\Theta' := Reduction (\Theta;\overline D);$
%        return $\CSP(\Theta;\overline D')$;
%    end if;
%    return $\CSPLinear(\Theta)$;
%end Function;
%
%Function $\CSPLinear(\Theta)$
%%    $\Theta_L = Factorize(\Theta)$;
%    $res:= CSPSolveLinear(\Theta)$;
%    if $res = \varnothing$ then return false; %no solutions of the system of linear equations
%
%    while $res$ has a solution
%        $Y:= ChooseIndependentVariables(\Theta)$.
%        % Let Y = \{y_1,\ldots,y_s\}.
%
%        Put $(a_1,\ldots,a_s) = (0,0,\ldots,0)$.
%        % we choose a solution corresponding to independent variables (a_1,a_2,\ldots,a_s)
%        $\widetilde S:= ChooseSolution(\Theta; res;(a_1,a_2,\ldots,a_s))$
%
%        if $\CSP(LinearReduction(\Theta,\widetilde S)) = true$ return true;
%        $\Theta' := \Theta$.
%1:
%        for each $\Omega\in SimplifiedCSP(\Theta')$
%            for each $i = 1$ to $s$
%                for each $a\in Dom(y_i)$
%                    $\widetilde S:= ChooseSolution(\Omega;\overline D; res;(a_1,a_2,\ldots,a_{i-1},a,a_{i+1},\ldots,a_{s}))$
%                    if $\CSP(LinearReduction(\Omega,\widetilde S)) = false$
%                        $\Theta' := \Omega$
%                        $a_{i} := a$
%                        Go to 1;
%                    end if
%                end for;
%            end for;
%        end for;
%        %Here we are in the position when every split gives a solution.
%        %Therefore all constraints are adjacent.
%        if $\Theta'$ is not linked
%            $res:= Add(res;CSPNotLinked(\Theta')).$
%        else
%            %Otherwise we search another equation in the form of $c_1 x_1 + c_2 x_2 + \ldots +c_n x_n = 1$
%            for each $i = 1$ to $s$
%                for each $a\in Dom(y_i)$
%                    $\widetilde S:= ChooseSolution(\Theta';\overline D; res;(a_1,a_2,\ldots,a_{i-1},a,a_{i+1},\ldots,a_{s}))$
%                    if $\CSP(LinearReduction(\Theta',\widetilde S)) = true$
%                        $c_{i} := 1/a (mod p)$
%                    end if
%                end for;
%            end for;
%            res := add(res,$c_1 x_1 + c_2 x_2 + \ldots +c_n x_n = 1$);
%        end if
%    end while;
%    % we are here only if res has no solutions.
%    % this means that we don't have a geberal solution
%    return false;
%end Function;

 

==> main_text_copy.tex <==

\section{Introduction}
\subsection{Constraint Satisfaction Problem}
The \emph{Constraint Satisfaction Problem (CSP)} is the problem of deciding whether there is an assignment to a set of variables
subject to some specified constraints. 
Formally, it can be defined in the following way.
Let $A$ be a finite set, 
$\Gamma$ be a set of relations on $A$, called 
a \emph{constraint language}.
Then \emph{the Constraint Satisfaction Problem over the constraint language} $\Gamma$, denoted by $\CSP(\Gamma)$, is
the following decision problem:
given a formula of the form 
$$R_{1}(z_{1,1},\dots,z_{1,n_1})\wedge
\dots
\wedge R_{s}(z_{s,1},\dots,z_{s,n_s}),
$$
where $R_{1},\dots,R_{s}\in\Gamma$ and each $z_{i,j}\in\{x_1,\dots,x_{n}\}$;
decide whether the formula is satisfiable.
It is well known that many combinatorial problems can be expressed as $\CSP(\Gamma)$
for some constraint language $\Gamma$.
Moreover, for some sets $\Gamma$ the corresponding decision problem can be solved in polynomial time;
while for others it is NP-complete.
It was conjectured in 1998 that
$\CSP(\Gamma)$ is either in P, or NP-complete \cite{FederVardi}.
In 2017 this conjecture was resolved independently 
by Andrei Bulatov \cite{BulatovProofCSP,bulatov2017dichotomy} and myself \cite{ZhukFOCSCSPPaper,MyProofCSP}. Moreover, the classification of the complexity for different constraint languages turned out to be very simple and was given in terms of polymorphisms.
We say that a $k$-ary operation $f$ is a \emph{polymorphism} of
an $m$-ary relation $R$
if 
whenever $(x^1_1,\ldots,x^m_1),\ldots,(x^1_k,\ldots,x^m_k)$ in $R$, then also $(f(x^1_1,\ldots,x^1_k),\ldots,f(x^m_1,\ldots,x^m_k))$ in $R$.
In this case we also say that $f$ \emph{preserves} $R$.
An operation $f$ is a \emph{polymorphism} of $\Gamma$ if it is a polymorphism of every relation in $\Gamma$.
An operation $w$ is called a \emph{weak near-unanimity (WNU) operation} 
if it satisfies the following identities
$$
w(y,x,\dots,x)=
w(x,y,x,\dots,x)=\dots = w(x,\dots,x,y).
$$
For instance a majority operation, conjunction, disjunction are WNU operations.
Then the complexity of $\CSP(\Gamma)$ is described by the following theorem.
%It was shown that $\CSP(\Gamma)$ is tractable if $\Gamma$ admits
%a WNU polymorphism, and it is NP-complete otherwise. 

\begin{thm}[\cite{BulatovProofCSP,bulatov2017dichotomy,ZhukFOCSCSPPaper,MyProofCSP}]\label{FederVardiConj}
Suppose $\Gamma$ is a finite constraint language on a finite set $A$.
Then $\CSP(\Gamma)$ is solvable is polynomial time 
if there exists a WNU polymorphism of $\Gamma$;
$\CSP(\Gamma)$ is NP-complete otherwise.
\end{thm}

\subsection{Surjective Constraint Satisfaction Problem}

In this paper we consider a variant of the CSP with an additional 
global constraint saying that a solution should be surjective.
\emph{The Surjective Constraint Satisfaction Problem over a constraint language $\Gamma$ on a domain $A$}, denoted by $\SCSP(\Gamma)$, is
the following decision problem:
given a formula of the form 
$$R_{1}(z_{1,1},\dots,z_{1,n_1})\wedge
\dots
\wedge R_{s}(z_{s,1},\dots,z_{s,n_s}),
$$
where $R_{1},\dots,R_{s}\in\Gamma$ and each $z_{i,j}\in\{x_1,\dots,x_{n}\}$;
decide whether there exists a solution
such that $\{x_{1},\dots,x_{n}\}=A$.
Unlike the complexity of the CSP, 
the complexity of $\SCSP(\Gamma)$ remains unknown even for very 
simple constraint languages $\Gamma$.

\subsection{Surjective Graph Homomorphism Problem}


Probably, the most natural examples of the Surjective CSP 
are defined as the graph homomorphism problem.
%The Surjective Constraint Satisfaction Problem is closely related to the surjective graph homomorphism problem.
%Assume that a graph $H$ is fixed, 
%for a given graph 
%$G$ we need to decide whether there exists a surjective 
%homomorphism from $G$ to $H$. 
%This problem is called \emph{the Surjective Graph Homomorphism Problem} and is denoted by $\SurjHom(H)$.
Assume that a graph $H$ is fixed, 
\emph{the Surjective Graph Homomorphism Problem}, denoted by $\SurjHom(H)$, is the problem of deciding 
for a given graph $G$ whether there exists a surjective 
homomorphism from $G$ to $H$. 
This problem is also known as 
\emph{the Vertex-Compaction Problem}
\cite{DBLP:journals/jda/Vikas18}
or \emph{the Surjective $H$-Colouring Problem} \cite{DBLP:journals/computability/GolovachJMPS19}.
For usual homomorphism this problem is known as
\emph{the $H$-colouring problem}.
Note that $\SurjHom(H)$ is equivalent 
to $\SCSP(\{H\})$, where the graph $H$ is viewed as a binary relation.


An interesting fact about the complexity of $\SurjHom(H)$ is that 
it remained unknown for many years even for very simple graphs $H$. 
Recall that the situation was different with the complexity of the CSP and the $H$-colouring problem: even though the general classification remained open for many years, nobody 
could show a simple constraint language or a graph with unknown complexity.
%see \cite{DBLP:journals/jct/MartinP15} for the reflexive 4-cycle and
%\cite{DBLP:conf/mfcs/Vikas17} for the 6-cycle. 
We will discuss two popular examples of such graphs.

First example is the complexity of $\SurjHom$ 
for the reflexive 4-cycle, which was formulated 
as an open question in \cite{dantas2005finding} and 
\cite{fleischner2009covering}, later
it was a principal open question in 
\cite{ito2011parameterizing,ito2011disconnected}, and the central question discussed in \cite{cook20102k2} and \cite{dantas20122k2}. 
This problem is known as \emph{the disconnected cut problem}, since it is equivalent to finding a cutset
(a set whose removal
results in a disconnected graph) such that the cutset is disconnected itself,
and it has attracted a lot of interest from the graph theory community. 
%This problem is considered important enough to generate its own complexity class \cite{de2012p,teixeira2011external}, and it is
This problem was 
known 
to be tractable for many graph classes \cite{cook20102k2,dantas20122k2,fleischner2009covering,ito2011parameterizing}, 
but in 2011 it was finally proved that  the disconnected cut problem is NP-complete \cite{DBLP:journals/jct/MartinP15}.

Second long-standing problem is 
the complexity of $\SurjHom$ 
for the non-reflexive 6-cycle, 
that has been of interest since 1999 \cite{vikas1999computational}
when Narayan Vikas proved 
NP-completeness of a similar problem for the 6-cycle, 
called \emph{the compaction problem}.
The difference between the compaction problem and the vertex-compaction problem is that for compaction we 
require the homomorphism to be edge-surjective.
In 2017 it was finally proved 
that $\SurjHom$ for the 6-cycle
is also NP-complete \cite{DBLP:conf/mfcs/Vikas17}.
It worth mentioning that 
the compaction and the vertex-compaction problems 
have the same complexity for all known graphs, and it was conjectured by Winkler, Vikas, and others that these problems are polynomially equivalent.
For more information about 
the relationship between 
the compaction problem and the vertex-compaction problem 
(and also the retraction problem) see \cite{DBLP:journals/jda/Vikas18}.



%For recent results on the complexity of $\SurjHom$ see \cite{DBLP:journals/toct/LaroseMP19,DBLP:journals/computability/GolovachJMPS19, DBLP:journals/siamdm/FockeGZ19}. 
Many other results on the complexity of 
$\SurjHom(H)$ can be found in 
\cite{DBLP:journals/toct/LaroseMP19,DBLP:journals/computability/GolovachJMPS19, DBLP:journals/siamdm/FockeGZ19,VikasOther, VikasIrreflexive,VikasReflexive,DBLP:journals/algorithmica/Vikas13,DBLP:journals/tcs/GolovachPS12,DBLP:conf/mfcs/Vikas17,DBLP:journals/jct/MartinP15}. For instance, 
the complexity of $\SurjHom$ 
is known
for all graphs on at most four vertices \cite{DBLP:journals/computability/GolovachJMPS19}.
But as far as we know the complexity remains unknown for graphs of size 5 and even for cycles, 
which makes this problem very intriguing because of the simplicity of the formulation. 




%In \cite{SCSPSURVEY} it was 



\subsection{The Complexity of SCSP}

Let us discuss what we know about the complexity of 
the SCSP and the CSP.
The complexity of $\CSP(\Gamma)$ is known for any constraint language $\Gamma$
\cite{BulatovProofCSP,bulatov2017dichotomy,ZhukFOCSCSPPaper,MyProofCSP}. The complexity of $\SCSP(\Gamma)$ 
is widely open.
Since we can always add dummy variables we never use and these dummy variables could give surjectivity,  $\CSP(\Gamma)$ can be trivially reduced to 
$\SCSP(\Gamma)$.
Also, it is sufficient to consider the reflexive 4-cycle $H$ to
get a constraint language $\Gamma=\{H\}$ such that 
$\SCSP(\Gamma)$ is NP-complete but 
$\CSP(\Gamma)$ is trivial and solvable in polynomial time.
Thus, sometimes $\SCSP(\Gamma)$ is harder than $\CSP(\Gamma)$.
%We know that sometimes $\SCSP(\Gamma)$ is NP-complete but 
%$\CSP(\Gamma)$ is trivial and solvable in polynomial time.

Another important observation is that 
$\SCSP(\Gamma)$ can be reduced to $\CSP(\Gamma\cup\{x=a\mid a\in A\})$ (see \cite[Section 2]{SCSPSURVEY}).
%In fact the reduction from $\SCSP(\Gamma)$ to %$\CSP(\Gamma\cup\{x=a\mid a\in A\})$ is known and %straightforward (see \cite[Section 2]{SCSPSURVEY}). 
Let us show how this reduction works.

\begin{lem}[\cite{SCSPSURVEY}]\label{SCSPTOCSP}
There exists a polynomial-time Turing reduction from $\SCSP(\Gamma)$ to $\CSP(\Gamma\cup\{x=a\mid a\in A\})$
\end{lem}
\begin{proof}
Let $A = \{a_1,\dots,a_{n}\}$. Suppose 
we have an instance $\mathcal I$ of 
$\SCSP(\Gamma)$.
First, we guess $n$ variables $x_{i_1},\dots,x_{i_n}$ such that these variables give all elements of $A$ in a solution, 
that is 
$x_{i_j}=a_j$ for every $j$.
Then we consider the following instance of $\CSP(\Gamma\cup\{x=a\mid a\in A\})$
$$\bigwedge\limits_{j=1}^{n}(x_{i_{j}} = a_{j})\wedge \mathcal I.$$
If it has a solution, then $\mathcal I$ has a surjective solution. 

Since we have only polynomially many choices for the 
variables, this gives us a polynomial-time Turing reduction to 
$\CSP(\Gamma\cup\{x=a\mid a\in A\})$.
\end{proof}

As a corollary we derive that 
$\CSP(\Gamma\cup\{x=a\mid a\in A\})$
and 
$\SCSP(\Gamma\cup\{x=a\mid a\in A\})$
are polynomially equivalent.

Recall that the classification of the complexity 
of the CSP for different constraint languages was given in terms of polymorphisms
(see Theorem \ref{FederVardiConj}).
It is natural to assume that the complexity of the SCSP can be 
described in a similar way.
In \cite{HubieSlides} Hubie Chen asked 
%not only this but also that 
whether 
Lemma~\ref{SCSPTOCSP} holds in both directions, which would imply 
the characterization of the complexity of SCSP in terms of polymorphisms.
Thus, he conjectured the following characterization of the complexity of 
$\SCSP(\Gamma)$.

\begin{conj}\label{HubieConj}
For any constraint language $\Gamma$ 
the problems 
$\CSP(\Gamma\cup\{x=a\mid a\in A\})$
and 
$\SCSP(\Gamma)$ 
are polynomially equivalent.
\end{conj}

An operation $f$ is called 
\emph{idempotent} if it satisfies 
$f(x,x,\dots,x) = x$.
Then, using Theorem \ref{FederVardiConj}
Conjecture \ref{HubieConj} can be formulated in the following form.

\begin{conj}\label{HubieConjTwo}
For any constraint language $\Gamma$ the problem $\SCSP(\Gamma)$ is solvable is polynomial time 
if there exists an idempotent WNU polymorphism of $\Gamma$;
$\SCSP(\Gamma)$ is NP-complete otherwise.
\end{conj}

As it was proved in \cite{SCSPforTwo1997} (see also \cite{SCSPforTwoBook}), Conjectures \ref{HubieConj} and \ref{HubieConjTwo}
hold for a 2-element domain. 
Also, all known results on the complexity of the 
SCSP agree with these conjectures (see \cite{SCSPSURVEY}).

Additionally, in \cite{chen2014algebraic} Hubie Chen confirmed that polymorphisms of $\Gamma$ can be used to 
describe the complexity of $\SCSP(\Gamma)$.
For instance, 
he proved NP-hardness of $\SCSP(\Gamma)$ for 
$\Gamma$ admitting only essentially unary polymorphisms.
For more results on the complexity of the SCSP see the survery 
\cite{SCSPSURVEY}.



\subsection{No Rainbow Problem}

In this paper we consider the most famous constraint language with 
unknown complexity of the SCSP.
Let $N =\{(a,b,c)\in\{0,1,2\}^{3}\mid \{a,b,c\}\neq\{0,1,2\}\}$. 
The problem $\SCSP(\{N\})$ is called \emph{No-Rainbow-Problem} 
and first appeared in \cite{ColoringMixedHypertrees}.
In fact, if we interpret 
$0,1$, and 2 as colors, then the relation $N$ forbids  
``rainbow''.
Despite the simplicity of the formulation, the complexity of $\SCSP(\{N\})$ 
was an open question for many years and was formulated 
many times as an important open problem 
\cite{SCSPSURVEY,HubieSlides}.
For example, Hubie Chen presented this 
problem as one of three concrete open questions 
at several conferences (see \cite{HubieSlides})
emphasizing that this problem is an important step 
toward a full classification of the complexity.

Note that the CSP 
over $N$ is trivial because 
any instance has a trivial solution 
where all variables are equal.
But if add all constant relations then 
the problem becomes 
NP-hard, that is 
$\CSP(\{N,x=0,x=1,x=2\})$ is NP-complete \cite{BulatovForThree}. 

As we mentioned in the previous subsection  $\SCSP(\{N,x=0,x=1,x=2\})$ is polynomially equivalent 
to $\CSP(\{N,x=0,x=1,x=2\})$.
It is interesting to compare the complexity of 
the CSP and the SCSP if we add some constant relations but probably not all of them.

$$\begin{array}{|c|c| c| c| c|}
\hline
  & \{N\} & \{N,x=0\} & \{N,x=0,x=1\}  & \{N,x=0,x=1,x=2\} \\ \hline
\CSP  & \text{P (Trivial)}     & \text{P (Trivial)}     & \text{ P (Trivial)}     & \text{NP-complete}     \\
\SCSP  & ???     & ???     & \text{NP-complete \cite{SCSPSURVEY}}     & \text{NP-complete}     \\
\hline
\end{array}$$

For instance, as it was shown in \cite{SCSPSURVEY}
if we add just two constant relations then 
the CSP is still trivial but 
the SCSP is already NP-complete. % (see the table above).
It can be shown that the only problems in the table with unknown complexity, that is  
$\SCSP(\{N\})$ and $\SCSP(\{N,x=0\})$, are polynomially equivalent. 
In fact, 
to reduce $\SCSP(\{N,x=0\})$ to $\SCSP(\{N\})$ 
we just replace all constraints $x_{i}=0$ by $x_{i}=z$ for a new variable $z$.


 \section{Main Results}\label{MainResultsSection}

In this section we formulate two main results of this paper. 

First, we proved that the No-Rainbow Problem is NP-hard, 
and therefore it is NP-complete.

\begin{thm}\label{NoRainbowTHM}
$\SCSP(\{N\})$ is NP-complete.
\end{thm}
Recently, Hubie Chen published a 
paper explaining the algebraic framework for proving such hardness results \cite{chen2020algebraic}.
He shows that this approach 
can also be used
to prove NP-hardness 
for the reflexive 4-cycle (the disconnected cut problem)
and for all NP-hard constraint languages on a 2-element domain.


Theorem \ref{NoRainbowTHM} agrees with Conjectures \ref{HubieConj} and \ref{HubieConjTwo}.
Unfortunately, we found a counter-example to these conjectures, which is the second main result of this paper.
Let us define 5-ary and 3-ary relations on the set $\{0,1,2\}$.
$$R = 
\begin{pmatrix}
0&0&0&0&0&0\\
2&2&2&1&1&1\\
2&1&1&1&1&1\\
1&2&2&1&1&1\\
0&1&2&0&1&2
\end{pmatrix}, R' = 
\begin{pmatrix}
2&2&1\\
2&1&1\\
1&2&1
\end{pmatrix}
\text{(here columns are tuples)}.$$
Note that $R'$ is the projection of $R$ onto coordinates 2, 3 and 4.
Hence, every polymorphism of $R$ is also a polymorphism of 
$R'$.

\begin{thm}\label{CEthm} We have
\begin{enumerate}
    \item[(1)] $\CSP(\{R,\{0\},\{1\},\{2\}\})$ is NP-hard.
    \item[(2)] $\SCSP(\{R\})$ is solvable in polynomial time.
    \item[(3)] $\SCSP(\{R'\})$ is NP-Hard.
\end{enumerate}
\end{thm}

Thus, items (1) and (2) of 
Theorem \ref{CEthm} disproves 
Conjectures \ref{HubieConj} and \ref{HubieConjTwo}. 
Also, comparing (2) and (3) we derive that 
the complexity of $\SCSP(\Gamma)$ cannot be described in terms of polymorphisms.
Hence, we need a brand new idea to describe the complexity of the SCSP for all constraint languages.

Nevertheless, our counter-example 
is of arity 5 and it is important for the proof.
Thus, probably for binary relations 
Conjectures \ref{HubieConj} and \ref{HubieConjTwo} still hold.
Another way to break our counter-example is 
to add all projections of relations from the constraint language to the constraint language. 
For instance, we could achieve this situation by considering only $\Gamma$ that are defined as the set of all invariants of some algebra, which is very natural way to define a constraint language for the CSP.
Thus, it is interesting to answer the following open questions.

\begin{problem}
Do Conjectures \ref{HubieConj} and \ref{HubieConjTwo} hold for 
$\Gamma = \{H\}$, where $H$ is a binary relation?
\end{problem}

\begin{problem}
Do Conjectures \ref{HubieConj} and \ref{HubieConjTwo} hold for 
$\Gamma$ consisting of binary relations?
\end{problem}

\begin{problem}
Do Conjectures \ref{HubieConj} and \ref{HubieConjTwo} hold for 
$\Gamma$ that is closed under projections (adding existential quantifiers)?
\end{problem}

For an algebra $\mathbf A = (A;f_1,f_{2},\dots)$
by $\Inv(\mathbf A)$ we denote the set of all relations
preserved by every operation $f_{i}$ of an algebra.

\begin{problem}
Do Conjectures \ref{HubieConj} and \ref{HubieConjTwo} hold for 
$\Gamma$ such that $\Gamma=\Inv(\mathbf A)$
for some algebra $\mathbf A$?
\end{problem}






The paper is organized as follows.
In Section \ref{FirstProofSection} and Section \ref{SecondProofSection} we give two different proofs 
of Theorem \ref{NoRainbowTHM}.
Both proofs are based on the reduction from an NP-hard CSP problem, 
the first reduction is easier in terms of complexity (just 2 variables for every variable of the original instance) but the idea of the reduction is hidden there.
We hope the second reduction is better for understanding
but there we create nine variables for every variable of the original instance.
In Section \ref{CounterExampleSection} we 
prove Theorem \ref{CEthm}.


\section{No-Rainbow problem is NP-Hard (the first proof)}
\label{FirstProofSection}

Here we present our first proof of the fact that $\SCSP(\{N\})$ is NP-hard.
By $[n]$ we denote the set $\{1,2,\dots,n\}$.
Let $\Gamma_{0} = \{x=y\vee z=0,x=y\vee z=1, x=0, x=1\}$ be a constraint language 
on $\{0,1\}$.
The problem $\CSP(\Gamma_{0})$ is known to be NP-Hard \cite{Schaefer}.
Hence, to prove Theorem \ref{NoRainbowTHM}
it is sufficient to 
prove the following theorem.

\begin{thm}\label{NoRainbowIsHard}
$\CSP(\Gamma_{0})$ can be polynomially reduced to $\SCSP(\{N\})$.
\end{thm}

Let us define the reduction. Let 
$\mathcal I$ be an instance of $\CSP(\Gamma_{0})$.
Let us build an instance $\mathcal J$ of $\SCSP(\{N,=\})$
such that $\mathcal I$ holds if and only if $\mathcal J$
has a surjective solution.
Note that 
the problems 
$\SCSP(\{N,=\})$
and 
$\SCSP(\{N\})$ are equivalent because we can always propagate out the equalities.

The idea is to introduce constraints (see 
$\mathcal C_{1},\mathcal C_{2},\dots, \mathcal C_{10}$ below) such that 
three concrete variables take all the values from the domain 
in any surjective solution. 
Below such variables are $x,x',y'$. 
Other variables still have some freedom, for instance $x_{1},\dots,x_{n}$ can be chosen 
freely from $\{x,x'\}$.
These variables will be used to encode 
the variables $u_{1},\dots,u_{n}$ of the instance $\mathcal I$.
By adding new constraints 
(see 
$\mathcal C_{11},\mathcal C_{12},\mathcal C_{13}, \mathcal C_{14}$ below)
we can encode constraints 
of $\CSP(\Gamma_{0})$ on the variables 
$x_{1},\dots,x_{n}$. A formal construction is below.




%By $S$ we denote 
%the relation defined by 
%$$S(v,v',t,t',z) = N(v,t,z)\wedge N(v',t,z)\wedge N(v,t',z)\wedge N(v',t',z).$$

\textbf{Construction}.
Let $u_{1},\dots,u_{n}$ be the variables of $\mathcal I$.

Choose variables $x,x',y',x_{1},\dots,x_{n},y_{1},\dots,y_{n},
z_{1},\dots,z_{n}$.
We define 14 sets of constraints:

\begin{itemize}
\item $\mathcal C_{1} = \{N(x,x_{i},y_{i})\mid i\in[n]\}$,

%$\mathcal C_{2} = \{S(x_{i},x',y_{i},y',z_{i})\mid i\in[n]\}$,
\item $\mathcal C_{2} = \{N(x',z_{i},y_{i})\mid i\in[n]\}$,

\item $\mathcal C_{3} = \{N(y',z_{i},x_{i})\mid i\in[n]\}$,

\item $\mathcal C_{4} = \{N(t_1,t_2,t_3)\mid 
t_{1},t_{2},t_{3}\in\{x,x',x_{1},\dots,x_{n}\}\}$,

\item $\mathcal C_{5} = \{N(t_1,t_2,t_3)\mid 
t_{1},t_{2},t_{3}\in\{x,y',y_{1},\dots,y_{n}\}\}$,

\item $\mathcal C_{6} = \{N(t_1,t_2,t_3)\mid 
t_{1},t_{2},t_{3}\in\{x',y',z_{1},\dots,z_{n}\}\}$,

\item $\mathcal C_{7} = \{N(x_{i},y_{j},z_{i})\mid 
i,j\in[n]\}$,

\item $\mathcal C_{8} = \{N(x_{i},y_{j},z_{j})\mid 
i,j\in[n]\}$,


\item $\mathcal C_{9} = \{N(x, x_{i},z_{i})\mid 
i,j\in[n]\}$,

\item $\mathcal C_{10} = \{N(x, y_{i},z_{i})\mid 
i,j\in[n]\}$,

\item $\mathcal C_{11} = \{N(x_{i}, x_{j},y_{k})\mid 
(u_{i}=u_{j}\vee u_{k} = 0)\in \mathcal I\}$,

\item $\mathcal C_{12} = \{N(y_{i}, y_{j},x_{k})\mid 
(u_{i}=u_{j}\vee u_{k} = 1)\in \mathcal I\}$,

\item $\mathcal C_{13} = \{x=x_{i}\mid 
(u_{i}=1)\in \mathcal I\}$,

\item $\mathcal C_{14} = \{x=y_{i}\mid 
(u_{i}=0)\in \mathcal I\}$.
\end{itemize}

\begin{lem}
$\mathcal I$ has a solution if and only if 
$\mathcal J$ has a surjective solution, where 
$\mathcal J = \mathcal C_{1}\cup\dots\cup \mathcal C_{14}$.
\end{lem}

\begin{proof}
Let us show both implications.

$\mathcal I\in\CSP(\Gamma_{0})\Rightarrow 
\mathcal J\in\SCSP(\{N,=\}).$

Let $(b_{1},\dots,b_{n})$ be a solution of $\mathcal I$.
Put 
$x = 1$, $x' = 0$, $y'=2$, 
$x_{i} = b_{i}$, $y_{i} = b_{i}+1$,
$z_{i} = 2\cdot b_{i}$ for every $i\in[n]$.
Let us check that all the constraints are satisfied.
\begin{itemize}
\item $\mathcal C_{1}$
holds because $|\{1,b_{i},b_{i}+1\}|<3$ for any $b_{i}\in\{0,1\}$.

\item $\mathcal C_{2}$
holds because 
$|\{0,2\cdot b_{i},b_{i}+1\}|<3$ for any $b_{i}\in\{0,1\}$.

\item $\mathcal C_{3}$
holds because 
$|\{2,2\cdot b_{i},b_{i}\}|<3$ for any $b_{i}\in\{0,1\}$.

\item $\mathcal C_{4}$
holds because 
$x,x',x_{1},\dots,x_{n}$ are from the set $\{0,1\}$.

\item $\mathcal C_{5}$
holds because 
$x,y',y_{1},\dots,y_{n}$ are from the set $\{1,2\}$.

\item $\mathcal C_{6}$
holds because 
$x',y',z_{1},\dots,z_{n}$ are from the set $\{0,2\}$.

\item $\mathcal C_{7}$
holds because $|\{b_{i},b_{j}+1,2\cdot b_{i}\}|<3$ for any $b_{i},b_{j}\in\{0,1\}$.

\item $\mathcal C_{8}$
holds because $|\{b_{i},b_{j}+1,2\cdot b_{j}\}|<3$ for any $b_{i},b_{j}\in\{0,1\}$.

\item $\mathcal C_{9}$
holds because $|\{1,b_{i},2\cdot b_{i}\}|<3$ for any $b_{i}\in\{0,1\}$.

\item $\mathcal C_{10}$
holds because $|\{1,b_{i}+1,2\cdot b_{i}\}|<3$ for any $b_{i}\in\{0,1\}$.

\item $\mathcal C_{11}$
holds because 
each constraint is equivalent 
to 
$|\{b_{i},b_{j},1+b_{k}\}|<3$ 
and 
equivalent to 
$(b_{i}=b_{j})\vee b_{k}=0$.

\item $\mathcal C_{12}$
holds because 
each constraint is equivalent 
to 
$|\{b_{i}+1,b_{j}+1,b_{k}\}|<3$ 
and 
equivalent to 
$(b_{i}=b_{j})\vee b_{k}=1$.

\item $\mathcal C_{13}$ holds because  
$x_{i} =x= 1$ whenever $b_{i} = 1$. 

\item $\mathcal C_{14}$ holds because  
$y_{i} =x=1$ whenever $b_{i} = 0$. 
\end{itemize}

$\mathcal J\in\SCSP(\{N,=\})\Rightarrow 
\mathcal I\in\CSP(\Gamma_{0}).$

Choose a surjective solution of $\mathcal J$. % and consider several cases. 
By $\mathcal C_{4}$ we can choose $a,b\in\{0,1,2\}$ such that 
$x=a$ and 
$\{x,x',x_{1},\dots,x_{n}\}\subseteq \{a,b\}$. 
Since the solution is surjective, there should be 
an element in the solution equal to $c\in\{0,1,2\}\setminus\{a,b\}$.
Consider 5 cases. 

\textbf{Case 1}. Assume that $y'=c$ and $x'=b$.
Note that by the definition of $N$ for any permutation $\sigma$ on $\{0,1,2\}$
$\sigma$ applied to a solution of an instance of $\SCSP(\{N\})$ gives a solution of the instance. Therefore, without loss of generality 
we may assime that 
%WLOG we may assume (everything is symmetric) that 
$x=1,x' = 0, y' = 2$ in our solution.
By $\mathcal C_{4}$,
$\mathcal C_{5}$,
$\mathcal C_{6}$
we know that 
$$\{x,x',x_{1},\dots,x_{n}\}=\{0,1\},\;
\{x,y',y_{1},\dots,y_{n}\}=\{1,2\},\;
\{x',y',z_{1},\dots,z_{n}\}=\{0,2\}.$$

Let us show that $y_{i} = x_{i}+1$.
If $x_{i} =0$ and $y_{i} = 2$, then we get a contradiction 
with $\mathcal C_{1}$.

If $x_{i} =y_{i} = 1$, then 
by $\mathcal C_{2}$ we have $z_{i}\neq 2$, 
by $\mathcal C_{3}$ we have $z_{i}\neq 0$,
which implies $z_{i}=1$ and contradicts $\mathcal C_6$.

Let us show that 
$(u_{1},\dots,u_{n}) = (x_{1},\dots,x_{n})$ is 
a solution of $\mathcal I$.

$\mathcal C_{11}$ guarantees that 
all the constraints of the form 
$(u_{i}=u_{j}\vee u_{k} = 0)$ hold, 
$\mathcal C_{12}$ guarantees that 
all the constraints of the form 
$(u_{i}=u_{j}\vee u_{k} = 1)$ hold, 
$\mathcal C_{13}$ guarantees that 
all the constraints of the form 
$u_{i}=1$ hold,
$\mathcal C_{14}$ guarantees that 
all the constraints of the form 
$u_{i}=0$ hold.
Thus, we proved that it is a solution.

\textbf{Case 2}. Assume that $y'=c$ and $x'=a$.
By $\mathcal C_{5}$
we have 
$\{x,y',y_1,\dots,y_n\}=\{a,c\}$.
By $\mathcal C_{6}$
we have 
$\{x',y',z_1,\dots,z_n\}=\{a,c\}$.
Since the solution is surjective, there should be $i$ 
such that $x_{i} = b$.
By $\mathcal C_{9}$ we have $z_{i}\neq c$,
by $\mathcal C_{3}$ we have $z_{i}\neq a$. Contradiction.

\textbf{Case 3}. Assume that $y'\neq c$ and $y_{i}=z_{i}=c$ for some $i$.
By $\mathcal C_{5}$
we have 
$\{x,y',y_1,\dots,y_n\}=\{a,c\}$, 
hence $y' = a$.
By $\mathcal C_{6}$
we have 
$\{x',y',z_1,\dots,z_n\}=\{a,c\}$, 
hence 
$x' = a$.
Since the solution is surjective, there should be $j$ 
such that $x_{j} = b$.
By $\mathcal C_{9}$, we have $z_{j} = a$.
By $\mathcal C_{7}$ 
we have $y_{\ell} = a$ for every $\ell$.
Contradiction.

\textbf{Case 4}. Assume that $y'\neq c$ and $y_{i}=c, z_{i}\neq c$ for some $i$.
By $\mathcal C_{5}$
we have 
$\{x,y',y_1,\dots,y_n\}=\{a,c\}$, 
hence $y' = a$.
By $\mathcal C_{1}$, we have 
$x_{i} = a$.
By $\mathcal C_{8}$ we obtain 
$z_{i}\in\{a,c\}$ and since $z_{i}\neq c$ we have
$z_{i} = a$.
Then by $\mathcal C_{8}$ we obtain 
$x_{\ell}=a$ for every $\ell$.
If $z_{j} = b$ for some $j$, then 
we get a contradiction with 
$\mathcal C_{7}$ applied to 
$(x_{j},y_{i},z_{j})$.
Since the solution is surjective, the only remaining option is 
$x'=b$, which contradicts 
$\mathcal C_{2}$.

\textbf{Case 5}. Assume that 
$\{x,y',y_1,\dots,y_n\}\subseteq\{a,b\}$.
Since the solution is surjective, 
there exists $i$ such that 
$z_{i} = c$.
By $\mathcal C_{9}$ and $\mathcal C_{10}$
we have $x_{i} = y_{i} = a$.
By $\mathcal C_{7}$ we have 
$y_{\ell} = a$ for every $\ell$,
by $\mathcal C_{8}$ we have 
$x_{\ell} = a$ for every $\ell$.
By $\mathcal C_{2}$ we have $x'\neq b$, 
by $\mathcal C_{3}$ we have $y'\neq b$.
Therefore $x'=y' = a$
and by $\mathcal C_{6}$
we obtain 
$\{x',y',z_1,\dots,z_n\}=\{a,c\}$.
Hence, none of the variables can be equal to $b$. Contradiction.
\end{proof}


\section{No-Rainbow problem is NP-Hard (the second proof)}\label{SecondProofSection}
Here we present another proof of the fact that 
the No-Rainbow problem is NP-Hard.
%Again, let $N =\{(a,b,c)\in\{0,1,2\}^{3}\mid \{a,b,c\}\neq\{0,1,2\}\}$.
By $NAE_{3}$ we denote the ternary relation 
on $\{0,1\}$ consisting of all tuples 
but $(0,0,0)$ and $(1,1,1)$.
The idea is to encode an instance 
of $\CSP(\{NAE_{3}\})$ using the relation $N$. 
We assign a binary operation 
on $A = \{0,1,2\}$ to every variable of the 
instance of $\CSP(\{NAE_{3}\})$ and then encode each binary operation with nine variables on $\{0,1,2\}$.
Our plan is to write conditions that guarantee 
that every binary operation depends essentially only on one variable.
Later we interpret the dependence on the first variable as $0$ and 
the dependence on the second variable as $1$.

It is known from \cite{Schaefer} that 
$\CSP(\{NAE_{3}\})$ is NP-hard. 
Hence, to prove Theorem \ref{NoRainbowTHM}
it is sufficient to reduce $\CSP(\{NAE_{3}\})$
to $\SCSP(\{N\})$.
We start with a few auxiliary facts.
For a relation $\rho$ by $\Pol(\rho)$ we denote the set of all polymorphisms of $\rho$.
We will need the following properties of $\Pol(N)$.

\begin{lem}[Section 5.2.6 in \cite{lau}]\label{SlupetskiClone}
Suppose $f\in \Pol(N)$ then 
\begin{enumerate}
    \item $f$ depends essentially only on one variable, or
    \item $|\Image(f)|<3$, that is, $f$ never returns some value
    $a\in A$.
\end{enumerate}
\end{lem}

We will encode each binary operation $f$ on $A$ via 
9 variables on $A$, which we denote by
%$$x_{0,0},x_{0,1},x_{0,2},
%x_{1,0},x_{1,1},x_{1,2},
%x_{2,0},x_{2,1},x_{2,2}.$$
$$
f(0,0), f(0,1),f(0,2),
f(1,0), f(1,1),f(1,2),
f(2,0), f(2,1),f(2,2).$$
For a tuple $\alpha$ by $\alpha(i)$ we denote the $i$-th element of this tuple. 
If we just write the definition of the fact that 
$f$ is a polymorphism of $N$ we get the following lemma.

\begin{lem}\label{PolWrittenAsConj}
$f\in \Pol(N)
\Leftrightarrow
\bigwedge_{\alpha,\beta\in N} 
    N(f(\alpha(1),\beta(1)),f(\alpha(2),\beta(2)),f(\alpha(3),\beta(3))).$$
$
%S(x_{0,0},x_{0,1},x_{0,2},
%x_{1,0},x_{1,1},x_{1,2},
%x_{2,0},x_{2,1},x_{2,2}) = \bigwedge_{\alpha,\beta\in N} 
%    N(x_{\alpha(1),\beta(1)},x_{\alpha(2),\beta(2)},x_{\alpha(3),\beta(3)}).$$
%    Then the tuples of $S$ represents all 
%    binary operations preserving $N$
\end{lem}

Thus, the condition $f\in\Pol(N)$ can be expressed as a 
conjunction of relations $N$. 

Now we are ready to prove the main theorem of this subsection.

\begin{thm}
$\CSP(\{NAE_{3}\})$ can be polynomially reduced to $\SCSP(\{N\})$.
\end{thm}

%First, let us define the reduction.
%For a relation $\rho$ by $\Pol(\rho)$ we denote the set of all polymorphisms of $\rho$.
%Note that 
%the relation $N$ defines a maximal clone
%of type $\mathcal B$, and 
%$\Pol(N)$ consists of all essentially unary operations, 
%and all operations $f$ such that $|\Image(f)|<3$
%(see Section 5.2.6 in \cite{lau}).

%Let $M$ be the matrix with 
%2 columns and $3^2=9$ rows whose rows are all pairs from 
%$\{0,1,2\}^{2}$.
%Let $S=\{f(M)\mid f\in\Pol(N)\}$, 
%that is, $S$ is the set of all graphs of binary operations from $\Pol(N)$.
%The fact that a binary operation 
%is a polymorphism of a relation can be easily expressed via a conjunctive formula over the relation, therefore, 
% $S$ can be defined 
%by a conjunctive (quantifier-free) formula over $\{N\}$.

%(About Section 3).
%    Let us show that being a polymorphism of $\rho$ of arity $h$ can be expressed via conjunctions.
%    Let $f$ be a binary operation, we want to express that $f$ preserves $\rho$.
%    We have a variable $x_{a,b}$ corresponding to the value $f(a,b)$.
%    Being a polymorphism means that 
%    for all $\alpha,\beta\in \rho$ we have 
%    $f(\alpha,\beta)\in \rho$. 
%    Then our conjunction is 
%    $$\bigwedge_{\alpha,\beta\in\rho} 
%    \rho(x_{\alpha(1),\beta(1)},x_{\alpha(2),\beta(2)},\dots,x_{\alpha(h),\beta(h)}).$$
%    (here by $\alpha(i)$ we mean the $i$-th element of $\alpha$).
%    In fact, this condition just says the definition of 
%    $f$ being a polymorphism of $\rho$.


Let us show how to encode $\CSP(\{NAE_{3}\})$ as 
$\SCSP(\{N\})$.
Consider an instance $\mathcal I$ of $\CSP(\{NAE_{3}\})$.
Let $x_{1},\dots,x_{n}$ be the variables 
of $\mathcal I$
and $T$ be the set of all triples 
$(i,j,k)$ such that 
$NAE_{3}(x_{i},x_{j},x_{k})$ appears in the instance.

As we mentioned earlier, we assign a binary operation $f_{i}$ on $A$ to each variable $x_{i}$, then we encode 
each operation with nine variables on $A$, which we denote by 
$f_{i}(0,0),f_{i}(0,1),f_{i}(0,2),$ 
$f_{i}(1,0)$, $f_{i}(1,1),$ $f_{i}(1,2),$ 
$f_{i}(2,0),$ $f_{i}(2,1),$ $f_{i}(2,2)$.

We want $f_{i}$ to depend only on the first variable
if $x_{i}=0$ and only on the second variable if $x_{i}=1$.
%To achieve this we do the following.
By $\mathcal I'$ we denote the following instance:
\begin{align*}
%\exists f_{1}\dots\exists f_n
&\bigwedge\limits_{i\in [n]}(f_{i}\in\Pol(N))
\bigwedge\limits_{i\in [n], a\in A}(f_{1}(a,a)=f_{i}(a,a))%\wedge
%\bigwedge\limits_{i,j\in[n],a,b\in A}N(f_{i}(a,b),f_{j}(a,b),f_{i}(a,a))
\bigwedge\limits_{(i,j,k)\in T}
N(f_{i}(0,1),f_{j}(1,2),f_{k}(2,0))\\
 &\bigwedge\limits_{i,j\in[n],a,b,c\in A}N(f_{i}(a,b),f_{i}(c,b),f_{j}(a,c))
  \bigwedge\limits_{i,j\in[n],a,b,c\in A}N(f_{i}(b,a),f_{i}(b,c),f_{j}(a,c))
 % \\
%   &\bigwedge\limits_{i,j\in[n],a,b,c\in A}N(f_{i}(a,b),f_{i}(c,b),f_{j}(c,a))
%    \bigwedge\limits_{i,j\in[n],a,b,c\in A}N(f_{i}(b,a),f_{i}(b,c),f_{j}(c,a))
\end{align*}
Note that by Lemma \ref{PolWrittenAsConj} the first conjunction 
can be written as a conjunction of relations $N$.
Hence, this instance can be viewed as an instance of 
$\SCSP(\{N\})$ because we use only equalities and the relation $N$
(the equations can be propagated out).

\begin{lem}
$\mathcal I$ has a solution if and only if 
$\mathcal I'$ has a surjective solution.
\end{lem}
\begin{proof}

$\mathcal I\Rightarrow \mathcal I'$.
Suppose we have a solution 
$(x_{1},\dots,x_{n})$ of $\mathcal I$. To get a surjective solution of $\mathcal I'$ it is sufficient to put
$f_{i}(x,y) = x$ if $x_{i} =0$ and
$f_{i}(x,y) = y$ if $x_{i} =1$.
Since $f_{i}(0,0) = 0$, 
$f_{i}(1,1) = 1$,
and
$f_{i}(2,2) = 2$ the solution is surjective.
Let us prove that all the above conjunctions hold.
The first conjunction holds since projections preserve
$N$. The second conjunction is trivial. The third conjunction holds because 
$(x_{1},\dots,x_{n})$ is a solution of $\mathcal I$
and therefore the operations $f_{i},f_{j},f_{k}$ cannot depend 
on the same variables. 
Let us check the fourth conjunction.
If $x_{i}=0$ then $f_{i}(a,b),f_{i}(c,b),
f_{j}(a,c)\in\{a,c\}$,
if $x_{i}=1$ then $f_{i}(a,b),f_{i}(c,b),
f_{j}(a,c)\in\{b,f_{j}(a,c)\}$.
The remaining conjunction can be verified in the same way. Thus, we get a surjective solution of $\mathcal I'$.

$\mathcal I'\Rightarrow \mathcal I$.
Suppose we have a surjective solution 
$(f_{1},\dots,f_{n})$ of $\mathcal I'$.
Let $g(x) := f_{1}(x,x)$.
By the second conjunction we have 
$f_{i}(x,x) = g(x)$ for every $i\in[n]$.

Assume that $|\Image(g)|=3$. By Lemma \ref{SlupetskiClone} 
each $f_{i}$ depends essentially only on one variable.  
%Moreover, since $|\Image(g)|=3$, it depends on this variable bijectively.
Assign $x_{i}=0$ if $f_{i}$ depends essentially on the first variable, 
and $x_{i}=1$ if $f_{i}$ depends essentially on the second variable. 
The third conjunction guarantees that 
$f_{i}, f_{j},$ and $f_{k}$ cannot depend on the same coordinate for each $(i,j,k)\in T$.
Indeed, if three operations $f_{i}, f_{j}, f_{k}$ 
depend only on the first variables then 
we get 
$$N(f_{i}(0,1),f_{j}(1,2),f_{k}(2,0)) = N(g(0),g(1),g(2)),$$ which does not hold because $g$ is a bijection. Thus, 
for each $(i,j,k)\in T$
we have $NAE_{3}(x_{i},x_{j},x_{k})$.
Hence, we defined a solution of $\mathcal I$.

Assume that $|\Image(g)|=2$. 
If $|\Image(f_{i})| =3$ for some $i$ then 
by Lemma \ref{SlupetskiClone} 
$f_{i}$ depends essentially only on one variable.
But this means that 
$\Image(f_{i}) = \Image(g)$, which gives a contradiction.
Hence
$\Image(f_{i})=\Image(g)$  for every $i\in[n]$, which contradicts the surjectivity of 
the solution.

Assume that $\Image(g)=\{d\}$. 
Assume that $|\Image(f_{k})|=3$ for some $k\in[n]$.
Then by Lemma~\ref{SlupetskiClone} $f_{k}$ depends essentially only on one variable and $\Image(f_{k})=\Image(g) = \{d\}$, which gives us a contradiction.
Thus, $|\Image(f_{k})|<3$ for every $k\in[n]$.
Since the solution is surjective, the remaining 
two values from $A\setminus\{d\}$ should appear in the images of some functions $f_{i}$ and $f_{j}$.
To get a contradiction we use the last two conjunctions. 
The fifth conjunction is obtained by a permutation of variables in 
$f_{i}$
from the fourth conjunction.
Therefore, without loss of generality
we consider 
$f_{i},f_{j}$ and $a,b,c\in A$ such that 
$\{d,f_{i}(a,b),f_{j}(a,c)\}=A$.
By the fourth conjunction we have 
$N(f_{i}(a,b),f_{i}(c,b),f_{j}(a,c))$, 
which together with $\Image(f_{i}) = \{f_{i}(a,b),d\}$
implies 
$f_{i}(c,b)= f_{i}(a,b)$. 
Then by the fifth conjunction we get 
$N(f_{j}(a,c), f_{j}(a,b), f_{i}(c,b))$
which together with $\Image(f_{j}) = \{f_{j}(a,c),d\}$
implies 
$f_{j}(a,b) = f_{j}(a,c)$.
Then by the fourth conjunction we have 
$(f_{i}(a,b),f_{i}(b,b),f_{j}(a,b))
= (f_{i}(a,b),d,f_{j}(a,c)) \in N$, which contradicts our assumption.
\end{proof}

==> preamble.tex <==

\section{Introduction}%

The \emph{Constraint Satisfaction Problem (CSP)} is the problem of deciding whether there is an assignment to a set of variables
subject to some specified constraints. 
%Many combinatorial problems can be expressed as constraint satisfaction problems 
%with some restri
Formally, the \emph{Constraint Satisfaction Problem} is defined as a triple $\langle \mathbf{X} , \mathbf{D} , \mathbf{C} \rangle$,
where
\begin{itemize}
\item
$\mathbf{X}=\{x_1,\ldots ,x_n\}$ is a set of variables,
\item
$\mathbf{D}=\{D_{1},\ldots ,D_{n}\}$ is a set of the respective domains,
\item
$\mathbf{C}=\{C_{1},\ldots ,C_{m}\}$ is a set of constraints,
\end{itemize}
where
each variable $x_{i}$ can take on values in the nonempty domain $D_{i}$,
every \emph{constraint} $C_{j}\in \mathbf{C}$ is a pair
$(t_{j},\rho_{j})$ where
$t_{j}$ is a tuple of variables of length $m_{j}$, called the \emph{constraint scope},
and $\rho_{j}$ is an $m_{j}$-ary relation on the corresponding domains,
called the \emph{constraint relation}.

The question is whether there exists \emph{a solution} to
$\langle \mathbf{X} , \mathbf{D} , \mathbf{C} \rangle$,
that is a mapping that assigns a value from $D_{i}$ to every variable $x_{i}$
such that
for each constraint $C_{j}$ the image of the constraint scope is a member of the constraint relation.

In this paper we consider only CSP over finite domains.
The general CSP is known to be NP-complete \cite{Num26, Num30}; however, certain restrictions
on the allowed form of constraints involved may ensure tractability (solvability in polynomial time)
\cite{Num4,Num20,Num22,Num23,CSPconjecture,BulatovAboutCSP}.
Below we provide a formalization to this idea.

To simplify the formulation of the main result we assume that the domain of every variable is a finite set $A$. 
Later we will assume that the domain of every variable is
a unary relation from the constraint language $\Gamma$
(see below).
%presentation we assume that
%all the domains $D_{1},\ldots,D_{n}$ are subsets of a finite set $A$.
By $R_{A}$ we denote the set of all finitary relations on $A$,
that is, subsets of $A^{m}$ for some $m$.
Thus, all the constraint relations are from $R_{A}$.

For a set of relations $\Gamma\subseteq R_{A}$ by $\CSP(\Gamma)$
we denote the Constraint Satisfaction Problem where all
the constraint relations are from $\Gamma$.
The set $\Gamma$ is called \emph{a constraint language}.
Another way to formalize the Constraint Satisfaction Problem is
via conjunctive formulas.
Every $h$-ary relation on $A$ can be viewed as
a predicate, that is, a
mapping $A^{h}\rightarrow \{0,1\}$.
Suppose $\Gamma\subseteq R_{A}$, then $\CSP(\Gamma)$ is the following decision problem:
given a formula
$$\rho_{1}(v_{1,1},\ldots,v_{1,n_{1}})
\wedge
\dots
\wedge
\rho_{s}(v_{s,1},\ldots,v_{s,n_{s}}),$$
where $\rho_{1},\dots,\rho_{s}\in \Gamma$, 
and $v_{i,j}\in \{x_{1},\dots,x_{n}\}$ for every $i,j$;
decide whether this formula is satisfiable.

It is well known that many combinatorial problems can be expressed as $\CSP(\Gamma)$
for some constraint language $\Gamma$.
Moreover, for some sets $\Gamma$ the corresponding decision problem can be solved in polynomial time;
while for others it is NP-complete.
It was conjectured that
$\CSP(\Gamma)$ is either in P, or NP-complete \cite{FederVardi}.

\begin{conj}\label{FederVardiConj}
Suppose $\Gamma\subseteq R_{A}$ is a finite set of relations.
Then $\CSP(\Gamma)$ is either solvable in polynomial time, or $NP$-complete.
\end{conj}

We say that an operation
$f\colon A^{n}\to A$ \emph{preserves} the relation $\rho\in R_{A}$ of arity $m$
if for any tuples $(a_{1,1},\ldots,a_{1,m}),\dots,(a_{n,1},\ldots,a_{n,m})\in \rho$
the tuple
$(f(a_{1,1},\ldots,a_{n,1}),\ldots,f(a_{1,m},\ldots,a_{n,m}))$ is in $\rho$.
We say that an operation \emph{preserves a set of relations $\Gamma$} if it preserves every relation in $\Gamma$.
A mapping $f:A\to A$ is called \emph{an endomorphism} of $\Gamma$ if it preserves $\Gamma$. %every relation $\rho\in \Gamma$.
%It can be shown

\begin{thm}\label{coreHasSameComplexity}\cite{jeavons1998algebraic}
Suppose $\Gamma\subseteq R_{A}$.
If $f$ is an endomorphism of $\Gamma$, %$f:A\to A$ preserves every relation of $\Gamma$,
then $\CSP(\Gamma)$ is polynomially reducible to $\CSP(f(\Gamma))$ and vice versa,
where $f(\Gamma)$ is a constraint language with domain $f(A)$
defined by $f(\Gamma) = \{f(\rho)\colon \rho\in \Gamma\}$.
\end{thm}

A constraint language is \emph{a core} if every endomorphism of $\Gamma$ is a bijection.
It is not hard to show that if $f$ is an endomorphism of $\Gamma$ with minimal range,
then $f(\Gamma)$ is a core. Another important fact is that we can add all
singleton unary relations to a core constraint language
without increasing the complexity of its $\CSP$.
By $\sigma_{=a}$ we denote the unary relation $\{a\}$.

\begin{thm}\label{addingIdempotency}\cite{CSPconjecture}
Let $\Gamma\subseteq R_{A}$ be a core constraint language, and
$\Gamma' = \Gamma\cup \{\sigma_{=a}\mid a\in A\}$.
Then $\CSP(\Gamma')$ is polynomially reducible to $\CSP(\Gamma)$.
\end{thm}
Therefore, to prove Conjecture~\ref{FederVardiConj} it is sufficient to consider only the case when
$\Gamma$ contains all unary singleton relations.
In other words, all the predicates $x = a$, where $a\in A$, are in the constraint language $\Gamma$.

In \cite{Schaefer} Schaefer
classified all tractable constraint languages over two-element
domain. In \cite{BulatovForThree} Bulatov generalized the result for three-element domain.
His dichotomy theorem was formulated in terms of a $G$-set.
Later, the dichotomy conjecture was formulated in several different forms (see \cite{CSPconjecture}).

The result of Mckenzie and Mar{\'o}ti~\cite{miklos} allows us to formulate the dichotomy conjecture in the following nice way.
An operation $f$ on a set $A$ is called \emph{a weak near-unanimity operation (WNU)} if it satisfies 
%$f(x,x,\ldots,x) = x$ and
$f(y,x,\ldots,x) = f(x,y,x,\ldots,x) = \dots = f(x,x,\ldots,x,y)$
for all $x,y\in A$.
An operation $f$ is called \emph{idempotent} if $f(x,x,\ldots,x) = x$ for all $x\in A$.

\begin{conj}\label{mainconj}
Suppose $\Gamma\subseteq R_{A}$ is a finite set of relations.
%$\{\sigma_{=a}\mid a\in A\} \subseteq \Gamma$.
Then $\CSP(\Gamma)$ can be solved in polynomial time if there exists a WNU
preserving $\Gamma$;
$\CSP(\Gamma)$ is NP-complete otherwise.
\end{conj}

It is not hard to see that
the existence of a WNU preserving $\Gamma$ is equivalent to the existence of
a WNU preserving a core of $\Gamma$,
and also equivalent to
the existence of an idempotent WNU preserving the core.
Hence, Theorems~\ref{coreHasSameComplexity} and \ref{addingIdempotency}
imply that it is sufficient to prove Conjecture~\ref{mainconj}
for a core and an idempotent WNU.

One direction of this conjecture follows from \cite{miklos}.
\begin{thm}\label{MiklosMckenzie}\cite{miklos}
Suppose $\Gamma\subseteq R_{A}$ and 
$\{\sigma_{=a}\mid a\in A\} \subseteq \Gamma$.
If there exists no WNU
preserving $\Gamma$, then $\CSP(\Gamma)$ is NP-complete.
\end{thm}

%%As it follows from Theorem~\ref{addingIdempotency} and Theorem~\ref{MiklosMckenzie},
%%to prove Conjecture~\ref{mainconj} it remains to
%%find a polynomial algorithm for constraint languages preserved by an idempotent WNU.

The dichotomy conjecture was proved for many special cases:
for CSPs over undirected graphs \cite{hell1990complexity},
for CSPs over digraphs with no sources or sinks \cite{barto2009csp},
for constraint languages containing all unary relations~\cite{bulatov2003conservative},
and many others.
%Recently, Rafiey, Kinne, and Feder
%announced the proof of the general case~\cite{PossibleProofCSP}.
More information about the algebraic approach to CSP can be found in \cite{bartopolymorphisms}.

In this paper we present an algorithm that
solves $\CSP(\Gamma)$ in polynomial time if $\Gamma$ is preserved by an idempotent WNU,
and therefore prove the dichotomy conjecture.

\begin{thm}
Suppose $\Gamma\subseteq R_{A}$ is a finite set of relations.
%$\{\sigma_{=a}\mid a\in A\} \subseteq \Gamma$.
Then $\CSP(\Gamma)$ can be solved in polynomial time if there exists a WNU
preserving $\Gamma$;
$\CSP(\Gamma)$ is NP-complete otherwise.
\end{thm}

Another proof of the dichotomy conjecture was announced by Andrei Bulatov~\cite{BulatovProofCSP,BulatovProofCSPFOCS}.
Even though both algorithms appeared at the same time, they are significantly different. 
Bulatov's algorithm uses full strength of the few subpowers algorithm \cite{idziak2010tractability}, 
uses Maroti's trick for trees on top of Mal'tsev \cite{maroti2011tree}, 
while this one just checks some local consistency and solves linear equations over prime fields. 
Also Bulatov's algorithm works for infinite constraint languages, which is not the case for the algorithm presented in this paper.
But its slight modification works even for infinite constraint languages \cite{zhuk2018modification}.


The paper is organized as follows.
In Section~\ref{ZFourExample} we explain the algorithm informally and 
give an example showing how the algorithm works
for a system of linear equations in $\mathbb Z_{4}$.
In Section~\ref{Definition} we give main definitions,
in Section~\ref{Algorithm}
we give a formal description of the algorithm
showing a pseudocode for most functions
and explain the meaning of every function.
In Section~\ref{CorretnessSection} we formulate all theorems 
that are necessary to prove the correctness of the algorithm.
Then, we prove that on every algebra (domain) with
a WNU operation 
there exists a subuniverse of one of four types, which is the main ingredient of the algorithm. 
Additionally, in this section we prove that 
some functions of the algorithm work properly 
and the algorithm actually works in polynomial time.

In Section~\ref{DefinitionSection} we give the remaining definitions.
The proof of the main theorems is divided into three sections.
In Section~\ref{AbsCenterPCLinear} we study  properties of
subuniverses of each of four types (absorbing, central, PC, and linear subuniverses).
In Section~\ref{AuxStatements} we prove all the auxiliary statements, and in the last section we prove the main theorems of this paper formulated in Section~\ref{CorretnessSection}.

In Section~\ref{ConclusionsSection}, 
we discuss open questions
and consequences of this result.
In particular, we consider generalizations 
of the CSP such as Valued CSP, Infinite Domain CSP, Quantified CSP, Promise CSP and so on.



%A CSP instance $\Theta$ is called \emph{1-consistent} if
%for any constraint $(t,R)$ the relation $R$ is subdirect.

%%%if the set of all variables that appears in $\Theta$
%%%can be divided into two sets $X_{1}$ and $X_{2}$ such that
%%%any constraint of $\Theta$ either has variables only from $X_{1}$
%%%or only from $X_{2}$.
%%%
%%%A CSP instance is called \emph{linked} if
%%%for any $i$ and $a,b\in A_{i}$ there exists a path $x_{i}-C_{1}-x_{i_1}-\dots-\dots-x_{i_l}-C_{l+1}-x_{i}$
%%%from $a$ to $b$.

%%A CSP instance $\Theta$ is called \emph{irreducible} if for
%%any nonlinked nontrivial subinstance $\Theta'$
%%,any variable $x_{i}$ that appears in $\Theta'$,
%%and any $a\in A_{i}$ we have a solution of $\Theta'$ with $x_{i} = a$.
%
%\section{Algorithm}
%
%Function $\CSP(\Theta)$
%    $PathConsistency(\Theta)$
%    $Irreducible(\Theta)$
%    If exists a proper binary absorbing set on $A_{i}$
%        $\overline D := MinimalAbsorbingSets(\Theta)$;
%        $\Theta' := Reduction (\Theta;\overline D);$
%        return $\CSP(\Theta;\overline D')$
%    end if;
%
%    If exists a proper center on $A_{i}$
%        $\overline D := MinimalCentralSets(\Theta)$;
%        $\Theta' := Reduction (\Theta;\overline D);$
%        return $\CSP(\Theta;\overline D')$;
%    end if;
%
%    If $A_{i}/\sigma$ is polynomially complete for some  $i$  and a congruence $\sigma$ on $A_{i}$
%        $\overline D := MinimalPCClasses(\Theta)$;
%        $\Theta' := Reduction (\Theta;\overline D);$
%        return $\CSP(\Theta;\overline D')$;
%    end if;
%    return $\CSPLinear(\Theta)$;
%end Function;
%
%Function $\CSPLinear(\Theta)$
%%    $\Theta_L = Factorize(\Theta)$;
%    $res:= CSPSolveLinear(\Theta)$;
%    if $res = \varnothing$ then return false; %no solutions of the system of linear equations
%
%    while $res$ has a solution
%        $Y:= ChooseIndependentVariables(\Theta)$.
%        % Let Y = \{y_1,\ldots,y_s\}.
%
%        Put $(a_1,\ldots,a_s) = (0,0,\ldots,0)$.
%        % we choose a solution corresponding to independent variables (a_1,a_2,\ldots,a_s)
%        $\widetilde S:= ChooseSolution(\Theta; res;(a_1,a_2,\ldots,a_s))$
%
%        if $\CSP(LinearReduction(\Theta,\widetilde S)) = true$ return true;
%        $\Theta' := \Theta$.
%1:
%        for each $\Omega\in SimplifiedCSP(\Theta')$
%            for each $i = 1$ to $s$
%                for each $a\in Dom(y_i)$
%                    $\widetilde S:= ChooseSolution(\Omega;\overline D; res;(a_1,a_2,\ldots,a_{i-1},a,a_{i+1},\ldots,a_{s}))$
%                    if $\CSP(LinearReduction(\Omega,\widetilde S)) = false$
%                        $\Theta' := \Omega$
%                        $a_{i} := a$
%                        Go to 1;
%                    end if
%                end for;
%            end for;
%        end for;
%        %Here we are in the position when every split gives a solution.
%        %Therefore all constraints are adjacent.
%        if $\Theta'$ is not linked
%            $res:= Add(res;CSPNotLinked(\Theta')).$
%        else
%            %Otherwise we search another equation in the form of $c_1 x_1 + c_2 x_2 + \ldots +c_n x_n = 1$
%            for each $i = 1$ to $s$
%                for each $a\in Dom(y_i)$
%                    $\widetilde S:= ChooseSolution(\Theta';\overline D; res;(a_1,a_2,\ldots,a_{i-1},a,a_{i+1},\ldots,a_{s}))$
%                    if $\CSP(LinearReduction(\Theta',\widetilde S)) = true$
%                        $c_{i} := 1/a (mod p)$
%                    end if
%                end for;
%            end for;
%            res := add(res,$c_1 x_1 + c_2 x_2 + \ldots +c_n x_n = 1$);
%        end if
%    end while;
%    % we are here only if res has no solutions.
%    % this means that we don't have a geberal solution
%    return false;
%end Function;



